Prioritized Multi-stream Traffic in Uplink IoT Networks: Spatially Interacting Vacation Queues

Massive Internet of Things (IoT) is foreseen to introduce plethora of applications for a fully connected world. Heterogeneous traffic is envisaged, where packets generated at each IoT device should be differentiated and served according to their priority. This paper develops a novel priority-aware spatiotemporal mathematical model to characterize massive IoT networks with uplink prioritized multistream traffic (PMT). Particularly, stochastic geometry is utilized to account for the macroscopic network wide mutual interference between the coexisting IoT devices. Discrete time Markov chains (DTMCs) are employed to track the microscopic evolution of packets within each priority stream at each device. To alleviate the curse of dimensionality, we decompose the prioritized queueing model at each device to a single-queue system with server vacation. To this end, the IoT network with PMT is modeled as spatially interacting vacation queues. Interactions between queues, in terms of the packet departure probabilities, occur due to mutual interference. Service vacations occur to lower priority packets to address higher priority packets. Based on the proposed model, dedicated and shared channel access strategies for different priority classes are presented and compared. The results show that shared access provides better performance when considering the transmission success probability, queues overflow probability and latency.

==> miscellaneous/biography.tex <==
\begin{IEEEbiography}
		[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{miscellaneous/Mustafa_Emara.jpg}}]
		{Mustafa Emara}(S’18) received his B.Sc. degree in communications engineering from the German University in Cairo (GUC) in 2014 and the M.Sc. from the Technical University in Munich in 2017. He is currently with the EU-wireless standards team, Next Generation and Standards, Intel Deutschland and pursuing his Ph.D. at the Institute of Communications, Hamburg University of Technology. Prior to that he was with Fraunhofer Heinrich Hertz Institute, Nomor Research and Telefonica Deutschland  as a student Researcher. He is the recipient of the Best Student Paper Award at the European Conference on Networks and Communications 2018. His research areas of interest include modeling of wireless communication systems, signal processing, and queueing theory.
	\end{IEEEbiography}

	\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{miscellaneous/Hesham_ElSawy.jpg}}]
		{Hesham ElSawy}(S’10–M’14–SM’17) is an assistant professor at King Fahd University of Petroleum and Minerals (KFUPM), Saudi Arabia. Prior to that, he was a postdoctoral Fellow at King Abdullah University of Science and Technology (KAUST), Saudi Arabia, a research assistant at TRTech, Winnipeg, MB, Canada, and a telecommunication engineer at the National Telecommunication Institute, Egypt. Dr. ElSawy received his Ph.D. degree in Electrical Engineering from the University of Manitoba, Canada, in 2014, where he received several academic awards, including the NSERC Industrial Postgraduate Scholarship during the period of 2010–2013, and the TRTech Graduate Students Fellowship in the period of 2010–2014. He co-authored three award-winning papers that are recognized by the IEEE COMSOC Best Survey Paper Award, the Best Scientific Contribution Award to the IEEE International Symposium on Wireless Systems 2017, and the Best Paper Award in Small Cell and 5G Networks (SmallNets) Workshop of the 2015 IEEE International Conference on Communications (ICC). He is the recipient of the IEEE ComSoc Outstanding Young Researcher Award for Europe, Middle East, $\&$ Africa Region in 2018. He is recognized as an exemplary reviewer by the IEEE Transactions on Communications for the three years 2014–2016, by the IEEE Transactions on Wireless Communications in 2017 and 2018, and by the IEEE Wireless Communications Letters in 2018. His research interests include statistical modeling of wireless networks, stochastic geometry, and queueing analysis for wireless communication networks.
	\end{IEEEbiography}

	\begin{IEEEbiography}	
		[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{miscellaneous/bauch.eps}}]
		{Gerhard Bauch}	received the Dipl.-Ing. and Dr.-Ing. degree in electrical engineering from Munich University of Technology (TUM), Munich, Germany, in 1995 and 2001, respectively, and the DiplomVolkswirt (master in economics) degree from Fern Universitaet Hagen, Hagen, Germany, in 2001. In 1996, he was with the German Aerospace Center, Oberpfaffenhofen, Germany. From 1996 to 2001, he was a Member of Scientific Staff with TUM. In 1998 and 1999, he was also a Visiting Researcher with AT$\&$T Labs Research, Florham Park, NJ, USA. In 2002, he joined DOCOMO Euro-Labs, Munich, Germany, where he has been managing the Advanced Radio Transmission Group. In 2007, he was additionally appointed a Research Fellow of DOCOMO Euro-Labs. He was a Full Professor with the Universitaet der Bundeswehr Munich from 2009 to 2012. Since October 2012, he has been the Head of the Institute of Communications, Hamburg University of Technology, Hamburg, Germany.
	\end{IEEEbiography}
	

==> simulation_results/figures/PMF_PAoI/1col/PMF_PAoI.tex <==
\definecolor{mycolor1}{rgb}{0.49020,0.18039,0.56078}%
\definecolor{mycolor2}{rgb}{0.39216,0.83137,0.07451}%

\begin{tikzpicture}[scale=0.9]
\begin{groupplot}[group style={
	group name=myplot,
	group size= 2 by 1,  horizontal sep=2cm}, height=1.5in,width=2.7in]
\nextgroupplot[title={{\smash{(a)}}},
scale only axis,
bar shift auto,
log origin=infty,
xmin=0.506666666666667,
xmax=9.49333333333333,
xtick={1, 2, 3, 4, 5, 6, 7, 8, 9},
xlabel style={font=\color{white!15!black}},
xlabel={Time slot},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={PMF},
axis background/.style={fill=white},
title style={font=\bfseries},
xmajorgrids,
ymajorgrids,
yminorgrids,]
\addplot[ybar, bar width=0.09, fill=red, draw=black, area legend] table[row sep=crcr] {%
	1	0.884179410263595\\
	3	0.0149105023308881\\
	5	0.000343463862117487\\
	7	7.91170022045798e-06\\
	9	1.82246248455508e-07\\
};


\addplot[ybar, bar width=0.09, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
	1	0.613549088960524\\
	3	0.0784372902648972\\
	5	0.0251669102589455\\
	7	0.00776143390003007\\
	9	0.00239712125293475\\
};


\addplot[ybar, bar width=0.09, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
	1	0.066800306872735\\
	3	0.0308713684813394\\
	5	0.0317002025595595\\
	7	0.0326398427742859\\
	9	0.0338031142773686\\
};


\addplot[ybar, bar width=0.09, fill=red, dashed, draw=black, area legend] table[row sep=crcr] {%
	1	0.832285593550967\\
	3	0.041485665893205\\
	5	0.00834899999070087\\
	7	0.00168023820623142\\
	9	0.000338148333072602\\
};


\addplot[ybar, bar width=0.09, fill=mycolor1, dashed, draw=black, area legend] table[row sep=crcr] {%
	1	0.410661764258016\\
	3	0.0949320714419968\\
	5	0.0569194457051267\\
	7	0.0361253415082518\\
	9	0.02326513000898\\
};


\addplot[ybar, bar width=0.09, fill=mycolor2, dashed, draw=black, area legend] table[row sep=crcr] {%
	1	0.00242661217712157\\
	3	0.00142595831395413\\
	5	0.0019374494474004\\
	7	0.0026768129146514\\
	9	0.00371769620774712\\
};



\nextgroupplot[title={{\smash{(b)}}},
scale only axis,
scale only axis,
xmin=-20,
xmax=0,
ymin=5,
ymax=20,
ylabel style={font=\color{white!15!black}},
ylabel={Peak age of information},
xlabel={$\theta$ [dB]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend columns=6,column sep=0.13cm, legend cell align=left, at={(-0.2,-0.35)},anchor=north}
]

\addlegendimage{style={color=red, line width=2.0pt}}
\addlegendentry{$i=1$}
\addlegendimage{style={color=mycolor1, line width=2.0pt}}
\addlegendentry{$i=2$}
\addlegendimage{style={color=mycolor2, line width=2.0pt}}
\addlegendentry{$i=3$}
\addlegendimage{style={color=black, line width=2.0pt}}
\addlegendentry{Shared}
\addlegendimage{style={color=black,dashed, line width=2.0pt}}
\addlegendentry{Dedicated-EA}
\addlegendimage{style={color=black, draw=none,mark size=3 pt, only marks, mark=*, mark options={solid, fill=green}}}
\addlegendentry{Overflow threshold}

%%%%%%%%%%%%%%%% shared %%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red, line width=2.0pt]
table[row sep=crcr]{%
	-20	11.0280779324822\\
	-19	11.0355463291185\\
	-18	11.0450597379202\\
	-17	11.0572148025451\\
	-16	11.0727956213618\\
	-15	11.0928415398277\\
	-14	11.1164792882261\\
	-13	11.1489632529324\\
	-12	11.1912142407668\\
	-11	11.1242778867137\\
	-10	11.1582058973641\\
	-9	11.2020001902684\\
	-8	11.2589076414607\\
	-7	11.3334829859066\\
	-6	11.4322675876701\\
	-5	11.5649181652435\\
	-4	11.7461529878801\\
	-3	11.9992445795701\\
	-2	12.3625750773541\\
	-1	12.9025817855138\\
	0	13.740859346535\\
};
\addplot [color=mycolor1, line width=2.0pt]
table[row sep=crcr]{%
	-20	5.27320411977801\\
	-19	5.28352164515196\\
	-18	5.29668926044659\\
	-17	5.31355398570157\\
	-16	5.33523898892559\\
	-15	5.36325000056504\\
	-14	5.39644244970271\\
	-13	5.44234610370865\\
	-12	5.50255825809183\\
	-11	5.40743213448983\\
	-10	5.45546868268737\\
	-9	5.51802204574688\\
	-8	5.60024195022151\\
	-7	5.70962309276985\\
	-6	5.85744413358183\\
	-5	6.06138837225203\\
	-4	6.35062508782679\\
	-3	6.77646639498822\\
	-2	7.43713132984276\\
};
\addplot [color=black, draw=none,mark size=3 pt, mark=*, mark options={solid, fill=green}, forget plot]
table[row sep=crcr]{%
	-2	7.43713132984276\\
};
\addplot [color=mycolor2, line width=2.0pt]
table[row sep=crcr]{%
	-20	5.34739926491898\\
	-19	5.37711415034492\\
	-18	5.41536684268328\\
	-17	5.46490750619172\\
	-16	5.52952929710244\\
	-15	5.61457573800464\\
};
\addplot [color=black, draw=none,mark size=3 pt, mark=*, mark options={solid, fill=green}, forget plot]
table[row sep=crcr]{%
	-15	5.61457573800464\\
};
%%%%%%%%%%%%%%%% dedicated %%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red, dashed, line width=2.0pt]
table[row sep=crcr]{%
	-20	11.0164272310928\\
	-19	11.0204402838456\\
	-18	11.0258330715683\\
	-17	11.0326834039616\\
	-16	11.1455697559916\\
	-15	11.185758687816\\
	-14	11.2378744603109\\
	-13	11.3059567422488\\
	-12	11.3957123555805\\
	-11	11.5153793490824\\
	-10	11.6771440659237\\
	-9	11.8995354439744\\
	-8	12.2116042381796\\
	-7	12.6604837754254\\
	-6	13.3256228177724\\
	-5	14.34679465004\\
	-4	15.9820356566491\\
	-3	18.7344392910406\\
};
\addplot [color=black, draw=none,mark size=3 pt, mark=*, mark options={solid, fill=green}, forget plot]
table[row sep=crcr]{%
	-3	18.7344392910406\\
};
\addplot [color=mycolor1, dashed, line width=2.0pt]
table[row sep=crcr]{%
	-20	5.27127986324817\\
	-19	5.28032612953254\\
	-18	5.29271427421285\\
	-17	5.3086540984745\\
	-16	5.43753493941235\\
	-15	5.49475105850316\\
	-14	5.56972878416546\\
	-13	5.66903131710212\\
	-12	5.80234735318658\\
	-11	5.98447862498388\\
	-10	6.23900716415297\\
	-9	6.60552332419832\\
	-8	7.1551272674639\\
};
\addplot [color=black, draw=none,mark size=3 pt, mark=*, mark options={solid, fill=green}, forget plot]
table[row sep=crcr]{%
	-8	7.1551272674639\\
};
\addplot [color=mycolor2,  dashed, line width=2.0pt]
table[row sep=crcr]{%
	-20	5.37376326472556\\
	-19	5.41002304731888\\
	-18	5.45764566806479\\
	-17	5.51943274619235\\
};
\addplot [color=black, draw=none,mark size=3 pt, mark=*, mark options={solid, fill=green}, forget plot]
table[row sep=crcr]{%
	-17	5.51943274619235\\
};
\end{groupplot}

\end{tikzpicture}
